Learning to Understand Goal Specifications by Modelling Reward

Recent work has shown that deep reinforcement-learning agents can learn to follow language-like instructions from infrequent environment rewards. However, this places on environment designers the onus of designing language-conditional reward functions which may not be easily or tractably implemented as the complexity of the environment and the language scales. To overcome this limitation, we present a framework within which instruction-conditional RL agents are trained using rewards obtained not from the environment, but from reward models which are jointly trained from expert examples. As reward models improve, they learn to accurately reward agents for completing tasks for environment configurations---and for instructions---not present amongst the expert data. This framework effectively separates the representation of what instructions require from how they can be executed. In a simple grid world, it enables an agent to learn a range of commands requiring interaction with blocks and understanding of spatial relations and underspecified abstract arrangements. We further show the method allows our agent to adapt to changes in the environment without requiring new expert examples.

==> recycling_bin.tex <==
%In a series of papers \citep{MacGlashan2015GroundingEC,Arumugam2018GroundingNL,williams2018learning}, Tellex and colleagues refine this idea of learning reward models for free form language instructions by learning a mapping between them and goals specified in a formal language which can be interpreted against the environment to define an MDP, thereby treating IRL as weakly-supervised semantic parsing. Again, this class of approaches assumes that there is a formal verification function which can eventually serve as a reward function for a particular instruction, rather than learning a instruction-conditional reward model which is free of this restriction.


%Dima: that must go to the related work
%To our knowledge, ours is the first work to apply an IRL-like method to instruction-following and highlight the generalization differences between the reward model (which is the reward model in our case) and the policy. 
